Unsupervised Adversarial Image Inpainting

We consider inpainting in an unsupervised setting where there is neither access to paired nor unpaired training data. The only available information is provided by the uncomplete observations and the inpainting process statistics. In this context, an observation should give rise to several plausible reconstructions which amounts at learning a distribution over the space of reconstructed images. We model the reconstruction process by using a conditional GAN with constraints on the stochastic component that introduce an explicit dependency between this component and the generated output. This allows us sampling from the latent component in order to generate a distribution of images associated to an observation. We demonstrate the capacity of our model on several image datasets: faces (CelebA), food images (Recipe-1M) and bedrooms (LSUN Bedrooms) with different types of imputation masks. The approach yields comparable performance to model variants trained with additional supervision.

==> chapters/old.tex <==
% XXXXXXXXXXXXXXX Begin remove XXXXXXXXXXXXXXX

% Due to the intrinsinc nature of the corruption process, a masked images introduce uncertainty on the missing pixels. A natural way to generate diverse and plausibles output, is to introduce a latent space $Z$ which contains the possible outputs not contained in the input image. During training, the learned generator attempts to pass enough information to the generator to resolve  ambiguities regarding the output. For example, if the generator is presented with a picture of a face with missing eyes, the vector $z \in Z$ represents the color of the eyes.

% A natural approach to allow the generator to extend its mapping to a latent vector $z$ is to learn the mapping $ G :  Y \times Z \rightarrow X $, where $z$ is drawn from a latent space with a standard gaussian prior. The generator is now a mapping between an corrupted input, a noise vector, and a sample from the true signal distribution. In theory, by sampling different $z \sim \rz$ we could generate multiple uncorrupted signal. 



% %------------------------------------------------------------------------

% % \subsubsection{Conditionning}
% % \label{sub:cond}
% In our setting, is it easy to see that the output of the generator is not conditioned on its input $y$ It has no reason to generate complete image whith pixel corresponding to the input image. Or it could chose to ignore the information from $y$ and produce sample from the input $z$. One simple workaround is given to us by the nature of the inpainting task.

% In this work, we assume that we can retrieve the mask $m$ trough the operator $T : Y \rightarrow M$.

% \begin{equation}
% \label{eq:mask_retrieval}
% m = T(y) 
% \end{equation}

% In practice, it consits in finding the pixels of $y$ which are equals to $\tau$ (in our case, $0$). We enforce the conditioning by computing :

% \begin{equation}
% \label{eq:generator}
%  \hat{x} = G(y, z) \odot \bar{m} + y
% \end{equation}

% This masking ensures of $G$ that the observed part of $y$ stays the same in the output of the generator. The loss is now :

% \begin{equation}
% % \begin{split}
%     \mathcal{L}^{GAN}(G, D) \defeq
%     \E_{\substack{\bar{y} \sim \P_\ry}} \big[ \log D(\bar{y}) \big] 
%     + \E_{\substack{y \sim \P_\ry \\ \hat{m} \sim \P_\rtheta \\ z \sim \P_z}} \big[ \log\big(1 - D(F[G(y, z)+y, \hat{m}]\big) \big]
% % \end{split}
%     \label{eq:adversarial_z_x}
% \end{equation}

% This loss is described in figure \ref{fig:gan_loss}.\\
% XXXXXXXXXXXXX End remove XXXXXXXXXX

% %Note that we are regressing over a point estimate of the latent $z$, whereras, in the previous lost, $E$ was producing a distrbution.                                                                                                                  
% \begin{figure}
% \begin{center}
% \includegraphics[width=0.95\textwidth]{images/attach_cvpr.pdf}
% \end{center}
%   \caption{The proposed model with the $z$ reconstruction loss. The generated masked images $\tilde{y=}F(G(y,z), \bar{m})$ is encoded into the latent vector $\tilde{z}$.}
% \label{fig:recon_loss}
% \end{figure}

% XXX la figure est à refaire en partie il y a un m de trop, c'est juste une modif de la figure et notations a revoir (tilde, hat)


% \begin{equation}
% % \begin{split}
%     \mathcal{L}^{rec_l}(G, D, E) \defeq
%     \E_{\substack{y \sim \P_\ry}} \big[ \log D(y) \big] 
%     + \E_{\substack{\tilde{y} \sim \P_\ry \\ m \sim \sim \P_m \\ \hat{z} \sim{E(y)}}} \big[ \log\big(1 - D(F[G(\tilde{y}, \hat{z}) + \tilde{y}), m]\big) \big]
% % \end{split} +
% \end{equation}

% \begin{equation}
%     \mathcal{L}^{enc_1 l_1}(G,E) \E_{\substack{y \sim \P_\ry \\ \hat{z} \sim z \\ m  \sim \p_m \\ z \sim{E(y)}}} \left\Vert y - \hat{y}\right\Vert_2^2
%     \label{eq:recon_1_1}
% \end{equation}


% \begin{equation}
%     \mathcal{L}^{enc_{kl}}(E) \E_{\substack{y \sim \P_\ry }} \ \KLD{E(y)}{\P_z}
% \label{eq:recon_kl}
% \end{equation}\\


% Equation \ref{eq:recon_1} is similar to equation \ref{eq:adversarial_z_x_1} with $\hat{z}$ infered from input $y$ and $\hat{z}$ and $\tilde{y}$ used as input for $G$. Equation \ref{eq:recon_1_1} forces the reconstruction of $y$ by this module and equation XXXla met-on ?\\

% XXXXXXXXXXXXXXXXXXXXXXXXXXX\\
% One way to force the latent code $z$ to be contain information is to map the input $Y$ to $z$ using the encoding function. The generator $G$ then uses both the latent code and an input image $\hat{y} = F(G(y, \hat{z}), \hat{m})$ to produce the desired reconstruction $\hat{x}$. By masking the $\hat{x}$ with the same mask $m = T(Y)$, $\tilde{y} = F(\hat{x}, m)$ should be indistinguable with $y$. Figure \ref{fig:kl_loss} illustrate this process.

% This loss can be seen as a variational autoencoder \cite{kingma2014adam} of $y$ with the latent code $z$ concatenated $\hat{y}$ in the middle. The conditional distribution $\P(z|y)$ is defined as $E(y)$. By sampling $z \sim E(y)$ we can write the loss : 

% \begin{equation}
% % \begin{split}
%     \mathcal{L}^{rec_D}(G, D, E) \defeq
%     \E_{\substack{\bar{y} \sim \P_\ry}} \big[ \log D(\bar{y}) \big] 
%     + \E_{\substack{y \sim \P_\ry \\ \hat{z} \sim \P_z \\ \hat{m} \sim \hat{m} \sim \P_\rtheta \\ z \sim{E(y)}}} \big[ \log\big(1 - D(F[G(\hat{y}, z)+\hat{y}, T(y)]\big) \big]
% % \end{split} +
%     \label{eq:recon_1}
% \end{equation}

% Where $\hat{y} = F[G(y, \hat{z})+ y, \hat{m}]$. Note that as $\hat{y}$ is also a function of $y$, one could argue that the reconstruction information is encoded in $\hat{Y}$ instead of of being encoded in $z$. However $y$ is masked by a random mask $\hat{m}$ forcing $z$ to encode some information on $Y$. As in \cite{zhu_toward_2017}, we also add a $l_1$ loss term to force similarity between $y$ and $\tilde{y}$ :  

% \begin{equation}
%     \mathcal{L}^{enc_1 l_1}(G,E) \E_{\substack{y \sim \P_\ry \\ \hat{z} \sim z \\ \hat{m} \sim \hat{m} \sim \P_\rtheta \\ z \sim{E(y)}}} \left\Vert Y - F[G(\hat{y}, z)+\hat{y}, T(y)]\right\Vert_2^2
%     \label{eq:recon_1_1}
% \end{equation}

% and the distribution $E(y)$ is encorouged te be close to a $\P_\rtheta$ with : 

% \begin{equation}
%     \mathcal{L}^{enc_{kl}}(E) \E_{\substack{y \sim \P_\ry }} \ \KLD{E(y)}{\P_z}
%     \label{eq:recon_kl}
% \end{equation}

% \\
% XXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXX

%------------------------------------------------------------------------

% The adversarial and encoding losses provide complementary strengths to our model : they allow the generator to inpaint images with plausible composition, and they map a latent vector to the reconstructed output . By combinining thoses losses, our final objective function is :


% $$ \mathcal{L}(G, D, E) = \mathcal{L}^{GAN}(G, D)  + \lambda \mathcal{L}^{enc}(G,E)$$ 

% Our model can be seen as an adapation of the principle of \cite{pajot_unsupervised_2019} and \cite{zhu_toward_2017}.

%We propose a pair of loss, that could force force the latent vector $z$ to be taken into account. We introduce the function $E : Y \rightarrow Z$, which encode the semantic information of a corrupted image $y$ into a latent code $z$.


%In order to lead the generator $G$ to produce sample from $\rx$, we adopt a adversarial approach similar with the one in AmbientGan \cite{ambientgan} and \cite{pajot_unsupervised_2019}.  In this model, a network $G$ map a corrupted samples $y = F(x, \theta)$ to the domain $X$ of uncorrupted images. 


%As we do not have access to sample from the ditribution $X$, we sample $\hat{m}$ from the $M$ distribution, and then apply transformation $\tilde{y} = F(\hat{x}, \hat{m})$. We use the discriminator $D$ to match sample from the original $y$ from the generated sample.
%Intuitively, this requires the network to \textit{remove} the corruption by producing samples that re-corrupted are indistiguishable from real corrupted sample. 
